A Load Balance Strategy for Hybrid Particle-Mesh Methods

We present a load balancing strategy for hybrid particle-mesh methods that is based on domain decomposition and element-local time measurement. This new strategy is compared to our previous approach, which assumes a constant weighting factor for each particle to determine the computational load. The timer-based load balancing is applied to a plasma expansion simulation. The performance of the new algorithm is compared to results presented in the past and a significant improvement in terms of computational efficiency is shown.

==> graphs/fig_gyrotron_initial_condition.tex <==
\begin{figure}[!h]
\sidecaption%[t]
\includegraphics[trim = 0mm 0mm 0mm 0mm, clip, width=11cm]{./graphs/gyrotron.png}
\caption{Grid and initial particle distribution for the gyrotron test case.}
\label{fig_gyrotron_initial_condition}
\end{figure}

==> gyrotron.tex <==
\subsection{Encountered Imbalances}

\input{./graphs/fig_gyrotron_initial_condition.tex}
The load-balancing algorithm is validated for a small setup, the simulation of a 
TE$_{2,3}$ gyrotron resonator, operating at \SI{30}{\giga\hertz}, which is used
as an academic  benchmark \cite{stock201201}. This setup is slightly modified,
a linear mesh with curvilinear boundaries consisting out of 
\num{2449} hexahedra is used. In each element,
the solution is approximated by a sixth order polynomial. All other parameters are 
identically. An element based domain-decomposition is used, thus only a limited number
of cores can be used for a balanced simulation. However, the setup inherit a strong
load imbalance. The particles are confined to a hollow electron beam, while all other
cells outside of the beam are empty. The setup can be regarded as stationary and is 
a good choice to emphasize the load imbalance.  \Figure~\ref{fig:te-load-distribution} depicts
the measured computational load for all elements after \SI{5}{\nano\second} simulation time.
The minimal required computational time is 
$t_\text{min}=\SI{7.44}{\second} $ compared to a maximum of $t_\text{max}=\SI{618.3}{\second} $, which leads
to a ratio of $R_\text{max/min}=83.03$ in the load per element. This means, that for this case, 
each particle laden element is up to 80 times more expensive than a particle free element. Furthermore, 
to account for one particle laden element, the next process would have to receive up to 80 elements to maintain
load balance. For the presented setup, only a small number of processes can be used until the 
total amount of load cannot be distributed homogeneously.  Please note, that this factor depends on the 
encountered number of particles inside each element and thus vary strongly between different elements and
simulations. If more particles would cluster inside an element, then the ratio would be higher, complicating 
the task of finding a good load balance or rendering it impossible.


\begin{figure}
  \scalebox{0.6}{\input{./graphs/te23_curved_2449elem_5ns.pgf}}
  \caption{Measured computational time for particle laden and particle free elements. The ratio between
           the maximal to minimal computational time is $80$.}
  \label{fig:te-load-distribution}
\end{figure}



